Unlocking Transfer Learning for Open-World Few-Shot Recognition

Few-Shot Open-Set Recognition (FSOSR) targets a critical real-world challenge, aiming to categorize inputs into known categories, termed closed-set classes, while identifying open-set inputs that fall outside these classes. Although transfer learning where a model is tuned to a given few-shot task has become a prominent paradigm in closed-world, we observe that it fails to expand to open-world. To unlock this challenge, we propose a two-stage method which consists of open-set aware meta-learning with open-set free transfer learning. In the open-set aware meta-learning stage, a model is trained to establish a metric space that serves as a beneficial starting point for the subsequent stage. During the open-set free transfer learning stage, the model is further adapted to a specific target task through transfer learning. Additionally, we introduce a strategy to simulate open-set examples by modifying the training dataset or generating pseudo open-set examples. The proposed method achieves state-of-the-art performance on two widely recognized benchmarks, miniImageNet and tieredImageNet, with only a 1.5\% increase in training effort. Our work demonstrates the effectiveness of transfer learning in FSOSR.

==> 0_abstract.tex <==
\begin{abstract}
Few-Shot Open-Set Recognition (FSOSR) targets a practical few-shot learning scenario, aiming to categorize inputs into known categories, termed closed-set classes, while simultaneously identifying open-set inputs that fall outside these classes. Previous efforts in the field have predominantly depended on prior knowledge from training datasets. However, our novel approach adopts transfer learning specifically tailored for FSOSR tasks. Given the scarcity of open-set examples in such tasks, we have formulated a two-stage method called Learning to Transfer Learning (LTL). This method involves open-set aware meta-learning and open-set free transfer learning. In the first stage, open-set aware meta-learning, we train a model to establish a metric space with a task-independent open-set representation, which serves as a beneficial starting point for the subsequent stage. In the second stage, open-set free transfer learning, the model, armed with its pre-established open-set representation, is further fine-tuned to adapt to a specific test task. For acquiring open-set examples during transfer learning, we either curate a training dataset, which is utilized in the first stage, or tailor closed-set examples to generate pseudo open-set examples. Then, our LTL achieves state-of-the-art performance across two widely recognized benchmarks, namely miniImageNet, and tieredImageNet. Our work represents significant advancements toward making transfer learning practically viable for FSOSR.
\end{abstract}

==> arxiv2/1_intro.tex <==
\vspace{-0.25cm}
\section{Introduction}
\label{sec:intro}
\vspace{-0.25cm}

Few-shot learning (FSL) has got a lot of attention due to the importance in enabling models to adapt to novel tasks using a few examples (e.g., $N$-way $K$-shot: a task involving $N$ distinct classes, each represented by $K$ examples)~\cite{FEAT,fsl_halluc,protonet,IER_distill,fastMAML,MAML}. However, in practical applications, FSL models inevitably encounter instances that do not belong to the $N$ classes, also known as open-set instances. Addressing this challenge has led to the emergence of the field of few-shot open-set recognition (FSOSR)~\cite{PEELER, snatcher_cvpr21, dprotonets, TANE, GEL}. 
% Within this context, the set of the $N$ known classes constitute a closed set, while the open set includes classes that are not part of the closed set.

\jtt{In FSOSR, if two $N$-way $K$-shot FSOSR tasks have distinct closed sets, their corresponding open sets will also differ. This interdependence presents a key challenge when adapting to novel tasks in FSOSR. Namely, it is essential to redefine not only the closed set but also the open set, since the open set is inherently shaped by its closed set.} Consequently, the open set lacks a universal definition across various FSOSR tasks; instead, it requires contextual consideration based on the closed set of a specific target task.

%\bg{One of the key challenges in FSOSR is that the open set is inherently dependent on its closed set, which varies across different few-shot scenarios. For instance, if two $N$-way $K$-shot FSOSR tasks have distinct closed sets, their corresponding open sets will also differ. Consequently, the open set lacks a universal definition across various FSOSR tasks; instead, it requires contextual consideration based on the closed set of a specific target task.}

% Notice that, in FSOSR, the definition of the open set is intrinsically linked to that of the closed set, thereby introducing specific challenges. For instance, if two $N$-way $K$-shot FSOSR tasks have distinct closed sets, their corresponding open sets also differ.
% Namely, the open set lacks a universal definition across various FSOSR tasks; rather, it necessitates contextual consideration relying on the closed set of a specific target task.

\begin{figure}[t]
    \centering
    %\includegraphics[width=\linewidth]{Figure/Intro4.png}
    % \includegraphics[width=\linewidth]{Figure/Intro2.pdf}
    % \includegraphics[width=\linewidth]{Figure/Intro3.pdf}
    %\includegraphics[width=1.0\linewidth]{Figure/Intro4.pdf}
    \includegraphics[width=0.7\linewidth]{Figure/Intro_v2.png}
    %\vspace{-0.1cm}
    %\caption{Accuracy-AUROC plot on \textit{mini}ImageNet (5-way 5-shot FSOSR). \jt{Open-set free} transfer learning only ($\Box$), \jt{Open-set aware} meta-learning only ($\bigtriangleup$), our complete LTL ($\largestar$). In ours, complete LTL  ($\largestar$) and its ablated are colored in red. LTL outperforms the recent SOTA for both accuracy and AUROC.} 
    \caption{\jtt{Difficulty of straightforward extension of the 
    %existing
    \bg{transfer learning from} FSL methods~\cite{IER_distill,fsl_halluc} to FSOSR. Compared to the pre-trained model without transfer learning (w/o TL), in open-set recognition, \cite{IER_distill,fsl_halluc} are less effective as much as in closed-set, or even degrade the performance.}} 
    \label{fig:intro}
    \vspace{-0.6cm}
\end{figure}

\bg{Despite recent advancements in the field, current works~\cite{PEELER, snatcher_cvpr21, dprotonets, TANE, GEL} have commonly focused on leveraging prior knowledge from a large training dataset. Then, they frequently struggle to balance closed-set accuracy with open-set recognition capabilities, often prioritizing open-set recognition at the expense of closed-set accuracy. Then, FSOSR research have faced saturated performance and struggled to achieve broad generalization across various benchmarks.}
% Previous works~\cite{PEELER, snatcher_cvpr21, dprotonets, TANE, GEL} in the field of FSOSR have commonly reliance on deriving prior knowledge favorable to FSOSR from a massive training dataset, from which the performance has reached a point of saturation \add{and presents challenges in achieving broad generalization across different benchmarks.} Moreover, a significant hurdle in FSOSR is balancing closed-set accuracy with open-set recognition capabilities. Previous efforts have tended to prioritize open-set recognition at the expense of closed-set accruacy.
% Whereas, 
In this work, we bring attention to the novel application of transfer learning within this field. Transfer learning~\cite{resnet, DeCAF, BERT, GPT} has been extensively studied and demonstrated its efficacy \add{leveraging a pre-trained model} to generalize 
% a model to 
\add{it to other} tasks.
Recent FSL methods~\cite{SKD, IER_distill, tian2020rethinking, fsl_halluc, felmi} have shown the efficacy of this approach.
\jtt{However, when they come to FSOSR, open-set examples are inherently not present, which significantly undermines the effect of transfer learning in terms of open-set recognition. Then, as in Fig.~\ref{fig:intro}, the naive extension of the transfer learning techniques of FSL, e.g. IER-distill~\cite{IER_distill} and Label Halluc.~\cite{fsl_halluc} fails to attain the same level of improvement in open-set recognition as seen in closed set, or even results in decreased result.}

%when they come to FSOSR, their pre-trained models are unable to impart the open-world knowledge. \add{Additionally, the absence of open-set examples for transfer learning further complicates the issue.} \add{Consequently, as described in Fig.~\ref{fig:intro},} the naive extension of the transfer learning techniques of FSL, e.g. IER-distill~\cite{IER_distill} and Label Halluc.~\cite{fsl_halluc}, to FSOSR is ineffective.

Tackling this point, we propose a two-staged FSOSR learning framework. Our method involves two stages: \textit{open-set aware meta-learning (\jtt{OAL}) and open-set free transfer learning (\jtt{OFL})}.
During the meta-learning stage, our objective extends beyond the meta-training of the feature encoder; we also aim to establish a universal open-set representation. This equips us with a decent starting point for the subsequent open-set free transfer learning.
In the transfer learning stage, we commence by initializing the model using the parameters obtained from the meta-learning stage. To counteract the absence of open-set examples, we develop two alternative open-set sampling strategies. The first approach curates a training dataset of the previous stage as a source of open-set examples for open-set free transfer learning.
For more pragmatic application, our second strategy is confined to the closed-set examples present in the target task, and exploits an episodic learning framework. \bg{Here, we generate \textit{pseudo} FSOSR episodes by randomly dividing the closed-set categories into a closed set and a pseudo open set.} 
% Here, we generate \textit{pseudo} FSOSR episodes by randomly selecting categories from the closed-set and designating them as `pseudo' open-set examples. Then, transfer learning can be conducted with only the curated episodes from the closed set, i.e. open-set example free.
% Both approaches are more favorable when built upon the initial meta-learning stage.
As a result, our \jtt{OAL-OFL} method attains a marked enhancement in performance metrics on the standard FSOSR benchmarks as depicted in Fig.~\ref{fig:intro} while incurring a minimal extra training expense of only 1.5\% compared to training without transfer learning. This allows \jtt{OAL-OFL} to surpass the existing state-of-the-art (SOTA) methods.

%\vspace{0.1cm}
\textbf{Our contributions}: \textbf{i)} We introduce a novel two-staged learning called \jtt{OAL-OFL}, bringing transfer learning to FSOSR for the first time with only a minimal additional cost. \textbf{ii)} We show the importance of preparing the model through open-set aware meta-learning, which is a sturdy starting point for transfer learning. \textbf{iii)} We suggest two breakthroughs to handle the lack of open-set examples during the transfer learning stage. \textbf{iv)} By leveraging the effectiveness of transfer learning, our proposed \jtt{OAL-OFL} achieves SOTA on \textit{mini}ImageNet and \textit{tiered}ImageNet datasets. This underscores its ability to generalize across various tasks, enhancing both closed-set classification accuracy and open-set recognition capabilities.
    % - areas where prior methodologies have struggled.

%\vspace{0.2cm}

\vspace{-0.15cm}
\section{Related Works} 
\vspace{-0.2cm}
\noindent \textbf{FSL}~\cite{FSL} can be streamlined into two approaches: meta-learning and transfer learning. Meta-learning, also known as learning-to-learn, can be categorized into optimization and metric-based methods. Optimization-based methods~\cite{MAML, prob_MAML, gradient-metalearn, fastMAML} involve training a meta-learner to adapt quickly to new tasks through a few optimization steps by learning adaptation procedures. 
In contrast, metric-based methods~\cite{poodle, protonet, matchingnet, FEAT} use a common feature embedding space where target classes of a new task can be distinguished using a distance metric. Recently, transfer learning-based approaches~\cite{SKD, IER_distill, fsl_halluc, felmi} have been suggested with superior results where a model trained on a large-scale base dataset is fine-tuned to a few-shot task with a small number of support examples. Our approach aligns with the transfer learning-based approaches of the few-shot classification, but transfer learning has yet to be explored in the context of FSOSR.

\noindent \textbf{OSR} aims to identify in-distribution samples within a closed set, and simultaneously detect the out-of-distribution samples from unseen classes. 
% The OOD samples can pose a challenge to classifiers, as they can be easily over-confidently classified as one of the closed categories \cite{foolDNN, OSR, OSR_survey}. 
% OSR was first introduced by \cite{OSR}, which used one-class or binary support vector machines to solve the problem. 
Early approaches focused on the confidence level and proposed various approaches such as using extreme value theory \cite{openmax, castillo2012extreme, generative_openmax, smith1990extreme}. Recently, there has been a growing interest in generative model-based approaches \cite{C2AE, gen_dis_OSR, conditional_gaussian_OSR}, which leverage the different reconstruction behavior between in-distribution and out-of-distribution samples. On the other hand, our method aligns more closely with distance-based approaches \cite{OSR_NN, metriclearning_OSR, reconstruction_OSR}, particularly those that specify open-set representation \cite{OSR_sota_22, masked_loss}.
% : Chen~\textit{et al.}~\cite{OSR_sota_22} used a reciprocal point for each closed-set class to represent open-set samples, while Zhou~\textit{et al.}~\cite{masked_loss} proposed reserving classifier placeholders for novel classes by augmenting the closed-set classifier with dummy classifiers. 
However, OSR methods assume the \add{distinct and fixed} class pools for the closed and open sets, which is not feasible in FSOSR, where both sets vary depending on a task. Then, it is hard to straightforwardly apply the conventional OSR methods to FSOSR.


\noindent \textbf{FSOSR.} Compared to few-shot classification and OSR, FSOSR has been less explored. PEELER~\cite{PEELER} introduced FSOSR task and aimed to maximize the entropy of open-set examples with Gaussian embeddings. They employed OSR approach~\cite{openmax} of detecting open-set examples based on the largest class probability. SnaTCHer~\cite{snatcher_cvpr21} used transformation consistency that similar examples remain closer after a set-to-set transformation.
% and detected open-set samples by distances before and after a transformation
%However, set-to-set function selection is required depending on the experimental setup. 
TANE~\cite{TANE} and D-ProtoNet~\cite{dprotonets} proposed a task-dependent open-set generator using support examples. %\bg{TODO:GEL~\cite{GEL}} 
Considering low-level features as well as semantic-level ones, GEL~\cite{GEL} designed a local-global energy score to measure the deviation of the input from the closed-set examples.
% Especially, TANE~\cite{TANE} achieved the SOTA performances with a transformer~\cite{transformer} attention block-based open-set prototype generator and detects open-set samples through the classification probability of the generated prototype. 
The aforementioned methods primarily employ the representative metric learning approach, ProtoNets~\cite{protonet}, and face difficulties in achieving generalization across diverse benchmarks. Our proposed approach, however, involves a two-stage learning process. The first stage focuses on meta-learning to train a task-independent open-set classifier that serves as an effective initialization for the second stage of transfer learning.
%\vspace{0.2cm}



==> arxiv2/2_method.tex <==

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/figure1_6.png}
    % \vspace{-0.8cm}
    \caption{
    \textbf{Overall training framework of OAL-OFL.} 
    % 새 그림의 경우
    \bg{(a) In Stage 1, the feature encoder and a learnable open-set prototype undergo distance-based meta-learning~\cite{protonet} with an additional class representing the open set. (b) In Stage 2, feature encoder and prototypes are further transfer-learned to the target task under an open-set-free condition. Open-set training examples can be alternatively drawn from the base training dataset (green) or from a subset of the closed-set categories that is randomly selected as a pseudo open set (purple).}
    % \bg{(a) In Stage 1, the feature encoder and a learnable open-set prototype undergo distance-based meta-learning~\cite{protonet} with an additional class representing the open set. (b) In Stage 2, the closed-set classifiers are initialized with their corresponding prototypes. The feature encoder and linear classifiers are transfer-learned to the target task under an open-set-free condition. Open-set training examples can be alternatively drawn from the base training dataset (blue) or from a subset of the closed-set categories (yellow) that is randomly selected as a pseudo open set.}
    % (a) In Stage-1, the feature encoder and a task-independent open-set prototype undergo \jt{open-set aware} meta-learning on training tasks sampled from the base training dataset. (b) In Stage-2, both the feature encoder and the open-set classifier are initialized from the meta-learned parameters. The close-set classifiers are initialized as their corresponding prototypes. Then, the feature encoder and linear classifiers are transfer-learned to the testing task, under the open-set free condition. To this end, open-set training examples can be alternatively drawn from the base training dataset (blue) when it is affordable for a ($N+1$)-way classification. Otherwise, a subset of the closed-set categories (yellow) is randomly selected to serve as pseudo open set training examples, not considering their true classes. In this example, one category is random-sampled as the pseudo open set, inducing an $N$-way classification.
    }    
    \label{fig:framework}
    \vspace{-0.4cm}
\end{figure*}

\vspace{-0.15cm}
\section{Proposed Method} 
\vspace{-0.3cm}
We present the proposed two-stage transfer learning process, dubbed OAL-OFL. The overall framework of OAL-OFL is depicted in Fig.~\ref{fig:framework}.
First, we describe the first stage, \jt{open-set aware} meta-learning, where a universal FSOSR metric space is obtained by learning the feature encoder and a \bg{learnable}
% task-independent
open-set prototype.
Then, we elaborate on the \jt{open-set free} transfer learning stage, especially suggesting two approaches to resolve the challenges of the absence of open-set examples.

\noindent\textbf{Problem definition.} \bg{The goal of FSOSR is two-fold: to classify an input query into one of the closed-set categories or to reject it as belonging to the associated open-set categories.} Formally, an $N$-way $K$-shot FSOSR task can be represented as $\mathcal{T}=\{S, Q, \tilde{Q}\ | \mathcal{C}, \Tilde{\mathcal{C}} \}$, where $C$ denotes a set of $N$ closed-set categories. The closed set is described by a support set $S$ which includes $K$ examples for each category, i.e. $\{x_i, y_i\}_1^{|S|}$ and $|S|=NK$. Here, $x$ represents the input data, while $y$ indicates its corresponding label. The query set for $C$ is denoted by $Q$. Distinctively, FSOSR also accommodates open-set queries $\tilde{Q}$, which belong to categories, $\Tilde{\mathcal{C}}$, that do not intersect with $C$ \bg{and are not explicitly defined.}
%. These $\Tilde{\mathcal{C}}$ means the open-set complement to $\mathcal{C}$, but not specified in both training and testing phases.

% \vspace{-0.15cm}
% \subsection{Stage-1: Meta-Learning FSOSR Metric Space}
\subsection{Stage-1: Open-set Aware Meta-Learning}
% \vspace{-0.15cm}
\vspace{-0.2cm}
We commence by meta-learning a metric space, which serves as a general starting point to tune the model to a specific target task in the \jt{open-set free} transfer learning of Stage-2.
As in Fig.~\ref{fig:framework} (a), this meta-learning stage involves the simultaneous training of the feature encoder $f_{\theta}$ and a \bg{learnable} 
% task-independent 
open-set prototype $c_\phi$. They are learned using FSOSR tasks drawn from the 
% large-scale 
base training dataset $\mathcal{D}_\rmbase$. \add{Though the definition of open set varies depending on $\mathcal{C}$, the $c_\phi$ is desired to be \bg{task-independent}
% universally represent an open-set class 
across $\forall \mathcal{C}$.} \add{Given the complexities involved in learning the task-specific open set classifier during Stage-2, the effective training of a reliable $c_\phi$ serves as a crucial link to bridge the two stages.}


In specific, given an $N$-way $K$-shot FSOSR task, $\mathcal{T}\sim \mathcal{D}_\rmbase$, \add{we conceptualize this as the $(N+1)$-way classification problem. In this framework, the $(N+1)$th class is designated as the open-set class.
For $n$-th class of $\mathcal{C}$, the classifier is formulated as the prototype $c_n$ which is defined as the mean feature vector over \bg{its} $K$ examples, i.e., $c_n=\frac{1}{K}\sum_{m=1}^{K}{f_\theta(x_m)}$~\cite{protonet}. Here, $f_\theta(x)$ produces a $D$-dimensional feature vector. Concurrently, for the open-set class, the corresponding classifier is characterized by the learnable open-set prototype $c_\phi$.}

Subsequently, the classification probability is
\begin{align}
\label{eq:stage1_class_prob}
    p(y=n|x) = &\frac{e^{-a\cdot d(c_\phi, f_{\theta}(x))+b}}{e^{-a\cdot d(c_\phi, f_\theta(x))+ b} + \sum_{n'=1}^{N}{e^{-d(c_{n'}, f_{\theta}(x))}}}
    & \text{if } n = N+1, \nonumber \\
    p(y=n|x) = &\frac{e^{-d(c_n, f_{\theta}(x))}}{e^{-a\cdot d(c_\phi, f_\theta(x))+ b} + \sum_{n'=1}^{N}{e^{-d(c_{n'}, f_{\theta}(x))}}}
     & \text{Otherwise},
\end{align}
where $d$ is a distance metric. Specifically, we use the squared Euclidean distance, $d(v, v') = ||v-v'||^2$. In addition, scalars $a$ and $b$ are also learned to calibrate the distance to $c_\phi$, inspired by D-ProtoNets~\cite{dprotonets}. This \add{calibration} enables that $c_\phi$ is solely accountable for representing open sets of \bg{various tasks.}
%all the FSOSR tasks. 
For the loss function, we utilize the cross-entropy (CE) loss which is formulated as:
\begin{align}
\label{eq:ce_loss}
\mathcal{L}_\textrm{CE}(x_i,y_i) = &-{\log{p_{\theta}(y=y_i|x_i)}}.
\end{align}
\bg{We further utilize the masked CE loss~\cite{masked_loss}, defined as: }
\begin{equation}
    \label{eq:mask_ce_loss}
    \mathcal{L}_\textrm{Mask}(x_i,y_i) = -{\log{p_{\theta\char`\\ y_i}(y=N+1|x_i)}},
\end{equation}
where $p_{\theta\char`\\ y_i}$ denotes the $N$-way classification probability, \bg{excluding the ground-truth label $y_i$. This loss term effectively creates pseudo open-set tasks by disregarding the true label. More precisely, }
%disregarding the ground-truth label, , i.e.,
\begin{equation}
\label{eq:prob_wo_target}
    p_{\theta\char`\\ y_i}(y=N+1|x_i) = \frac{e^{-d_{N+1}}}{e^{-d_{N+1}} + \sum_{n'=1, n'\neq y_i}^{N}{e^{-d(c_{n'}, f_{\theta}(x_i))}}}\nonumber,
\end{equation}
where we let $d_{N+1}=a\cdot d(c_\phi, f_{\theta}(x_i))+b$ for brevity.
% By disregarding the ground-truth class of the closed-set query, $\mathcal{L}_\textrm{Mask}$ allows for the treatment of $Q$ as open-set queries.

Overall, we learn $f_\theta$, $c_\phi$, $a$, and $b$ as
\begin{align}
    \label{eq:stage1_overall_loss}
    \theta^*_1, &\phi^*_1, a^*_1, b^*_1  = \argmin_{\theta,\phi, a, b} \{\mathbb{E}_{x\in \tilde{Q}}\mathcal{L}_{\textrm{CE}}(x, N+1)
    +\mathbb{E}_{(x,y)\in Q}\{\mathcal{L}_{\textrm{CE}} (x, y) + \mathcal{L}_{\textrm{Mask}} (x, y)\}\}.
\end{align}

% \vspace{-0.15cm}
% \subsection{Stage-2: Transfer Learning}
\subsection{Stage-2: Open-set Free Transfer Learning}
\label{subsubsec:stage2}
 \vspace{-0.2cm}
In this stage, we consider a target task, denoted as \add{$\mathcal{T}_\rmtest = \{S_\rmtest, Q_\rmtest, \tilde{Q}_\rmtest \ | \mathcal{C}_\rmtest, \Tilde{\mathcal{C}}_\rmtest \}$,} which is also configured as an $N$-way $K$-shot task. \add{Note that $Q_\rmtest$ and $\tilde{Q}_\rmtest$ are utilized solely for the purposes of inference during test.} The initial values of the learnable parameters are inherited from results of Stage-1. Specifically, $f_\theta$, $a$ and $b$ are imprinted as $f_{\theta^{*}_1}$, $a^{*}_1$ and $b^{*}_1$, respectively. We aim to train \add{them} alongside $(N+1)$-way classifiers. These classifiers are represented as $\{w_1, \cdots, w_{N+1}\}$, where each \add{$w_n \in \mathbb{R}^{D}$}. The first $N$ classifiers are set as the prototypes of the corresponding classes in $C_\rmtest$. The open-set classifier $w_{N+1}$ is initialized using $c_{\phi_{1}^{*}}$.

To ensure consistency with the meta-learned metric space, we compute the classification probability of each query based on the Euclidean distance as in \add{Eq.}~(\ref{eq:stage1_class_prob}). Then, during the transfer learning, we optimize $f_\theta$ and the classifier $g_\psi=\{w_1, \cdots, w_{N+1}, a, b\}$.

Since $\mathcal{T}_\rmtest$ lacks cues to learn the open-set classifier $w_{N+1}$, we suggest two approaches: i) sampling from the base training dataset $\mathcal{D}_\rmbase$ of Stage-1, and ii) sampling from the closed set $C_\rmtest$ of $\mathcal{T}_\rmtest$ itself.


\vspace{-0.15cm}
\subsubsection{Open-set sampling from base training dataset}
\vspace{-0.15cm}
Notice that \add{in the context of FSL,} the closed-set categories $C_\rmtest$ in $\mathcal{T}_\rmtest$ are exclusive with $\mathcal{D}_\rmbase$. As a result, we can exploit $D_\rmbase$ as a pool of open-set examples for $\mathcal{T}_\rmtest$.
Specifically, as in the green-colored of Fig.~\ref{fig:framework}(b), we randomly select $M$ examples from $\mathcal{D}_\rmbase$ at every iteration of the transfer learning to serve as open-set examples.

Then, the model is optimized as:
\begin{align}
\label{eq:transfer_CEloss}
\theta^*_2, \psi^*_2 =&\argmin_{ \theta, \psi}\{\mathbb{E}_{(x,y)\in S_\rmtest}\mathcal{L}_\text{CE}(x, y)
 + \mathbb{E}_{x\sim D_\rmbase}\mathcal{L}_\text{CE}(x, N+1)\}.
\end{align}

We call this unified process of Stage-1 and 2 with the base training dataset as \textit{OAL-OFL}. In the following section, we will introduce the OAL-OFL with a more practical open-set sampling, dubbed \textit{OAL-OFL-Lite}.

\vspace{-0.15cm}
\subsubsection{Pseudo open-set sampling from closed set}
\vspace{-0.15cm}
In real-world scenarios, $\mathcal{T}_\rmtest$ encompasses various categories, and we cannot guarantee that the closed set $C_\rmtest$ is not overlapped with the categories of $\mathcal{D}_\rmbase$. Additionally, after the meta-learning stage, the large-scale $\mathcal{D}_\rmbase$ may not be affordable due to practical constraints. To address these issues, we introduce OAL-OFL-Lite which operates with no necessity of $\mathcal{D}_\rmbase$.

Our strategy is the episodic random class sampling from the closed set $C_\rmtest$ itself to learn the open set. As exemplified in the purple-colored of Fig.~\ref{fig:framework}(b), we iteratively partition $C_\rmtest$ into the mutually exclusive subsets $\Acute{C}_\rmtest$ and $\Tilde{C}_\rmtest$. Subsequently, their corresponding support sets $\Acute{S}_\rmtest$ and $\Tilde{S}_\rmtest$ extracted from $S_\rmtest$ are used to transfer-learn the closed and open sets, % of \add{the modified task, $\Acute{\mathcal{T}}_\rmtest$,} 
respectively. Hence, we call $\Tilde{C}_\rmtest$ pseudo open set. Through this iterative pseudo open-set sampling, we can effectively learn the open-set classifier as well as the closed-set ones. Then, the model is optimized by the CE losses as
\begin{align}
\label{eq:transfer_CEloss_pseudo}
\theta^*_2, \psi^*_2 =&\argmin_{ \theta, \psi}\{\mathbb{E}_{(x,y)\in \Acute{S}_\rmtest}\mathcal{L}_\text{CE}(x, y) + \mathbb{E}_{x\in \Tilde{S}_\rmtest}\mathcal{L}_\text{CE}(x, |\Acute{C}_\rmtest|+1)\}.
\end{align}
where the open set is mapped to $(|\Acute{C}_\rmtest|+1)$th class and detected by $w_{N+1}$ in every iteration.
Moreover, we empirically found that the open-set representation tends to be overfitted to a testing task in OAL-OFL-Lite. Hence, we freeze %$c_{N+1}$ 
$w_{N+1}$ once it is initialized by the $c_{\phi_{1}^{*}}$. For more comprehensive understanding, we include Algorithm~\ref{alg:OAL-OFL} in Appendix.



==> arxiv2/3_exp.tex <==
\begin{table}[t] % Changed [t] to [htbp] for better float placement flexibility
    \caption{
        \textbf{Comparative results on the \textit{mini}ImageNet and \textit{tiered}ImageNet.} Averages of Acc (\%) and AUROC (\%) over 600 tasks are reported with 95\% confidence interval (*: reproduced, ${}^{\dagger}$: from \cite{snatcher_cvpr21}). For each case, bold and underlined scores indicate the best and second-best results.}
    \label{table:main_result} % Changed label slightly
    \centering
    \renewcommand{\arraystretch}{1.0}
    % Resizebox likely needed due to increased width. Adjust width (e.g., \linewidth, 0.9\linewidth) as needed.
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccc} % 1 method column + 4 for miniImageNet + 4 for tieredImageNet
    \toprule
    % --- Header Rows ---
    % Row 1: Dataset Names (Methods spans 3 rows)
    \multirow{3}{*}{\textbf{Methods}} & \multicolumn{4}{c}{\textbf{\textit{mini}ImageNet}} & \multicolumn{4}{c}{\textbf{\textit{tiered}ImageNet}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} % Rules under dataset names
    % Row 2: Shot counts
     & \multicolumn{2}{c}{\textbf{1-shot}} & \multicolumn{2}{c}{\textbf{5-shot}} & \multicolumn{2}{c}{\textbf{1-shot}} & \multicolumn{2}{c}{\textbf{5-shot}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} % Rules under shot counts
    % Row 3: Metrics
     & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC \\
    \midrule
    % --- Data Rows ---
    % Note: Using \scriptsize for confidence intervals for potentially better fit
    ProtoNets\cite{protonet}${}^{\dagger}$ & 64.01 \scriptsize{$\pm$0.9} & 51.81 \scriptsize{$\pm$0.9} & 80.09 \scriptsize{$\pm$0.6} & 60.39 \scriptsize{$\pm$0.9} & 68.26 \scriptsize{$\pm$1.0} & 60.73 \scriptsize{$\pm$0.8} & 83.40 \scriptsize{$\pm$0.7} & 64.96 \scriptsize{$\pm$0.8} \\
    FEAT~\cite{FEAT}${}^{\dagger}$ & 67.02 \scriptsize{$\pm$0.9} & 57.01 \scriptsize{$\pm$0.8} & 82.02 \scriptsize{$\pm$0.5} & 63.18 \scriptsize{$\pm$0.8} & 70.52 \scriptsize{$\pm$1.0} & 63.54 \scriptsize{$\pm$0.7} & 84.74 \scriptsize{$\pm$0.7} & 70.74 \scriptsize{$\pm$0.8} \\
    PEELER~\cite{PEELER}${}^{\dagger}$ & 65.86 \scriptsize{$\pm$0.9} & 60.57 \scriptsize{$\pm$0.8} & 80.61 \scriptsize{$\pm$0.6} & 67.35 \scriptsize{$\pm$0.8} & 69.51 \scriptsize{$\pm$0.9} & 65.20 \scriptsize{$\pm$0.8} & 84.10 \scriptsize{$\pm$0.7} & 73.27 \scriptsize{$\pm$0.7} \\
    SnaTCHer-F~\cite{snatcher_cvpr21} & 67.02 \scriptsize{$\pm$0.9} & 68.27 \scriptsize{$\pm$1.0} & 82.02 \scriptsize{$\pm$0.5} & 77.42 \scriptsize{$\pm$0.7} & 70.52 \scriptsize{$\pm$1.0} & 74.28 \scriptsize{$\pm$0.8} & 84.74 \scriptsize{$\pm$0.7} & 82.02 \scriptsize{$\pm$0.6} \\
    SnaTCHer-T~\cite{snatcher_cvpr21} & 66.60 \scriptsize{$\pm$0.8} & 70.17 \scriptsize{$\pm$0.9} & 81.77 \scriptsize{$\pm$0.5} & 76.66 \scriptsize{$\pm$0.8} & 70.45 \scriptsize{$\pm$1.0} & 74.84 \scriptsize{$\pm$0.8} & 84.42 \scriptsize{$\pm$0.7} & 82.03 \scriptsize{$\pm$0.7} \\
    SnaTCHer-L~\cite{snatcher_cvpr21} & 67.60 \scriptsize{$\pm$0.8} & 69.40 \scriptsize{$\pm$0.9} & 82.36 \scriptsize{$\pm$0.6} & 76.15 \scriptsize{$\pm$0.8} & \underline{70.85} \scriptsize{$\pm$1.0} & 74.95 \scriptsize{$\pm$0.8} & 85.23 \scriptsize{$\pm$0.6} & 80.81 \scriptsize{$\pm$0.7} \\
    ATT~\cite{TANE} & 67.64 \scriptsize{$\pm$0.8} & 71.35 \scriptsize{$\pm$0.7} & 82.31 \scriptsize{$\pm$0.5} & 79.85 \scriptsize{$\pm$0.6} & 69.34 \scriptsize{$\pm$1.0} & 72.74 \scriptsize{$\pm$0.8} & 83.82 \scriptsize{$\pm$0.6} & 78.66 \scriptsize{$\pm$0.7} \\
    ATT-G~\cite{TANE} & 68.11 \scriptsize{$\pm$0.8} & 72.41 \scriptsize{$\pm$0.7} & 83.12 \scriptsize{$\pm$0.5} & 79.85 \scriptsize{$\pm$0.6} & 70.58 \scriptsize{$\pm$0.9} & 73.43 \scriptsize{$\pm$0.8} & 85.38 \scriptsize{$\pm$0.6} & 81.64 \scriptsize{$\pm$0.6} \\
    GEL~\cite{GEL} & 68.26 \scriptsize{$\pm$0.9} & \underline{73.70} \scriptsize{$\pm$0.8} & 83.05 \scriptsize{$\pm$0.6} & \underline{82.29} \scriptsize{$\pm$0.6} & 70.50 \scriptsize{$\pm$0.9} & \underline{75.86} \scriptsize{$\pm$0.8} & 84.60 \scriptsize{$\pm$0.7} & 81.95 \scriptsize{$\pm$0.7} \\
    \cmidrule{1-9} % Separator rule spanning all columns
    \textbf{OAL-OFL} & \textbf{69.78} \scriptsize{$\pm$0.8} & \textbf{73.88} \scriptsize{$\pm$0.7} & \underline{85.49} \scriptsize{$\pm$0.7} & \textbf{83.13} \scriptsize{$\pm$0.6} & \textbf{71.73} \scriptsize{$\pm$0.5} & \textbf{75.88} \scriptsize{$\pm$0.6} & \textbf{86.75} \scriptsize{$\pm$0.6} & \textbf{83.36} \scriptsize{$\pm$0.6} \\
    \textbf{OAL-OFL-Lite} & \underline{69.15} \scriptsize{$\pm$0.8} & 72.21 \scriptsize{$\pm$0.9} & \textbf{85.61} \scriptsize{$\pm$0.6} & 81.11 \scriptsize{$\pm$0.6} & 70.80 \scriptsize{$\pm$0.9} & 73.67 \scriptsize{$\pm$0.7} & \underline{86.66} \scriptsize{$\pm$0.6} & \underline{82.22} \scriptsize{$\pm$0.6} \\
    \bottomrule
    \end{tabular}
    } % End resizebox
    \vspace{-0.5cm} % Keep original vertical space adjustment
\end{table}


\vspace{-0.15cm}
\section{Experimental Results}
\vspace{-0.2cm}
\subsection{Implementation Details}
\label{subsec:implementation}
\vspace{-0.2cm}
In line with established FSOSR approaches~\cite{PEELER, snatcher_cvpr21, TANE, GEL}, we conducted experiments using ResNet12~\cite{resnet12_mod} as the feature encoder on \textit{mini}ImageNet~\cite{matchingnet} and \textit{tiered}ImageNet \cite{tieredImageNet} benchmarks, with pre-training of the feature encoder accomplished on the corresponding base training dataset for each benchmark through the well-known FSL method, FEAT~\cite{FEAT}.
\textit{Mini}ImageNet is comprised of 100 categories each with 600 examples. These categories are divided into 64, 16, and 20 classes for training, validation, and testing purposes, respectively~\cite{ravi_split_iclr17}. \textit{Tierd}ImageNet consists of 608 categories and a total of 779,165 samples, which are divided into 351, 97, and 160 classes for training, validation, and testing, respectively. More training details are in Appendix.

%\noindent\textbf{Pretrain encoder.} In line with recent advancements in few-shot classification and FSOSR methods~\cite{fsl_halluc, snatcher_cvpr21, TANE}, we pretrained the encoder, $f_\theta$, using a linear classifier classifying all the classes in $\mathcal{D}_\text{Base}$. The encoder is trained for ? epochs with the SGD optimizer with cross-entropy loss, self-knowledge distillation~\cite{selfdistill}, rotation loss~\cite{TANE} with data augmentation using mixup~\cite{mixup}.


% \begin{table*}[t]
%     \caption{
%     \textbf{Comparative results on the \textit{mini}ImageNet and \textit{tiered}ImageNet.} Averages of Acc (\%) and AUROC (\%) over 600 tasks are reported with 95\% confidence interval (*: reproduced numbers, ${}^{\dagger}$: results from \cite{snatcher_cvpr21}). For each case, bold and underlined scores indicate the best and second-best results.}
%     \vspace{-0.2cm}
%     \label{table:main_result}
%     \centering
%     \renewcommand{\arraystretch}{1.0}
%     \resizebox{0.65\linewidth}{!}{
%     \begin{tabular}{llccccc}
%     \toprule

%     \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Methods}} &\multicolumn{2}{c}{\textbf{1-shot}} && \multicolumn{2}{c}{\textbf{5-shot}}\\
%     \cmidrule{3-4} \cmidrule{6-7}
%     & & Acc. & AUROC && Acc. & AUROC\\
%     \midrule
%     \midrule
%     \multirow{11}{*}{\textit{mini}ImageNet} & ProtoNets\cite{protonet}${}^{\dagger}$ & 64.01 \small{$\pm$ 0.9} & 51.81 \small{$\pm$ 0.9} && 80.09 \small{$\pm$ 0.6} & 60.39 \small{$\pm$ 0.9} \\
%     & FEAT~\cite{FEAT}${}^{\dagger}$ & 67.02 \small{$\pm$ 0.9} & 57.01 \small{$\pm$ 0.8} && 82.02 \small{$\pm$ 0.5} & 63.18 \small{$\pm$ 0.8}\\
%     & PEELER~\cite{PEELER}${}^{\dagger}$ & 65.86 \small{$\pm$ 0.9} & 60.57 \small{$\pm$ 0.8} && 80.61 \small{$\pm$ 0.6} & 67.35 \small{$\pm$ 0.8}\\
%     & SnaTCHer-F~\cite{snatcher_cvpr21} & 67.02 \small{$\pm$ 0.9} & 68.27 \small{$\pm$ 1.0} && 82.02 \small{$\pm$ 0.5} & 77.42 \small{$\pm$ 0.7}\\
%     &SnaTCHer-T~\cite{snatcher_cvpr21} & 66.60 \small{$\pm$ 0.8} & 70.17 \small{$\pm$ 0.9}&&81.77 \small{$\pm$ 0.5} &76.66 \small{$\pm$ 0.8}\\
%     &SnaTCHer-L~\cite{snatcher_cvpr21} & 67.60 \small{$\pm$ 0.8}&69.40 \small{$\pm$ 0.9}&&82.36 \small{$\pm$ 0.6} &76.15 \small{$\pm$ 0.8}\\
%     & ATT~\cite{TANE} & 67.64 \small{$\pm$ 0.8} & 71.35 \small{$\pm$ 0.7} && 82.31 \small{$\pm$ 0.5} & 79.85 \small{$\pm$ 0.6}\\
%     & ATT-G~\cite{TANE} & 68.11 \small{$\pm$ 0.8} & 72.41 \small{$\pm$ 0.7} && 83.12 \small{$\pm$ 0.5} & 79.85 \small{$\pm$ 0.6}\\
%     & GEL~\cite{GEL} & 68.26 \small{$\pm$ 0.9} & \underline{73.70} \small{$\pm$ 0.8} && 83.05 \small{$\pm$ 0.6} & \underline{82.29} \small{$\pm$ 0.6} \\
    
%     \cmidrule{2-7}
%     %\textbf{ASOP (Ours)} & 66.30 \small{$\pm$ 0.6} & \underline{71.72} \small{$\pm$ 0.5} && \underline{82.68 \small{$\pm$ 0.2}} & \underline{80.92 \small{$\pm$ 0.2}} && 68.68 \small{$\pm$0.7} & {74.92 \small{$\pm$ 0.4}} && 84.84 \small{$\pm$ 0.4} & \textbf{82.37 \small{$\pm$ 0.3}} \\ % 0.1, 0.5, 0.4
    
%     %\textbf{ASOP-L (Ours)} & \textbf{67.85 \small{$\pm$ 0.2}} & \textbf{71.91 \small{$\pm$ 0.7}} && \textbf{82.81 \small{$\pm$ 0.3}} & \textbf{81.04 \small{$\pm$ 0.2}} && \textbf{71.49} \small{$\pm$ 0.4} & \textbf{75.04} \small{$\pm$ 0.4} && \underline{85.15} \small{$\pm$ 0.1} & 81.51 \small{$\pm$ 0.1}\\
%     %\textbf{Stage-1} & 67.95 & 71.81 && 82.76 & 80.91 && 71.17 & 74.57 && 84.75 & 81.34 \\
%     & \textbf{OAL-OFL} & \textbf{69.78} \small{$\pm$ 0.8} & \textbf{73.88} \small{$\pm$ 0.7} && \underline{85.49} \small{$\pm$ 0.7} & \textbf{83.13} \small{$\pm$ 0.6}\\
    
%     & \textbf{OAL-OFL-Lite} & \underline{69.15} \small{$\pm$ 0.8} & 72.21 \small{$\pm$ 0.9} && \textbf{85.61} \small{$\pm$ 0.6} & 81.11 \small{$\pm$ 0.6}\\    
    
%     % \textbf{ASOP-F (Ours)} & 67.23 \small{$\pm$ 0.6} & 72.02 \small{$\pm$0.3} && 82.60 \small{$\pm$0.2} & 81.69 \small{$\pm$0.4}\\
    
%     \midrule
%     \multirow{11}{*}{\textit{tiered}ImageNet} & ProtoNets\cite{protonet}${}^{\dagger}$& 68.26 \small{$\pm$ 1.0} & 60.73 \small{$\pm$ 0.8} && 83.40 \small{$\pm$ 0.7} & 64.96 \small{$\pm$ 0.8}  \\
%     & FEAT~\cite{FEAT}${}^{\dagger}$ & 70.52 \small{$\pm$ 1.0} & 63.54 \small{$\pm$ 0.7} && 84.74 \small{$\pm$ 0.7} & 70.74 \small{$\pm$ 0.8}\\
%     & PEELER~\cite{PEELER}${}^{\dagger}$ & 69.51 \small{$\pm$ 0.9} & 65.20 \small{$\pm$ 0.8} && 84.10 \small{$\pm$ 0.7} & 73.27 \small{$\pm$ 0.7}\\
%     & SnaTCHer-F~\cite{snatcher_cvpr21} & 70.52 \small{$\pm$ 1.0} & 74.28 \small{$\pm$ 0.8} && 84.74 \small{$\pm$ 0.7} & 82.02 \small{$\pm$ 0.6}\\
%     &SnaTCHer-T~\cite{snatcher_cvpr21} & 70.45 \small{$\pm$ 1.0} & 74.84 \small{$\pm$ 0.8} && 84.42 \small{$\pm$ 0.7} & 82.03 \small{$\pm$ 0.7} \\
%     &SnaTCHer-L~\cite{snatcher_cvpr21} & \underline{70.85} \small{$\pm$ 1.0} & 74.95 \small{$\pm$ 0.8} && 85.23 \small{$\pm$ 0.6} & 80.81 \small{$\pm$ 0.7}\\
%     & ATT~\cite{TANE} & 69.34 \small{$\pm$ 1.0} & 72.74 \small{$\pm$ 0.8} && 83.82 \small{$\pm$ 0.6} & 78.66 \small{$\pm$ 0.7}\\
%     & ATT-G~\cite{TANE} & 70.58 \small{$\pm$ 0.9} & 73.43 \small{$\pm$ 0.8} && 85.38 \small{$\pm$ 0.6} & 81.64 \small{$\pm$ 0.6}\\
%     & GEL~\cite{GEL} & 70.50 \small{$\pm$ 0.9} & \underline{75.86} \small{$\pm$ 0.8} && 84.60 \small{$\pm$ 0.7} & 81.95 \small{$\pm$ 0.7} \\
%     \cmidrule{2-7}
%     & \textbf{OAL-OFL} & \textbf{71.73 }\small{$\pm$ 0.5}  & \textbf{75.88 }\small{$\pm$ 0.6} && \textbf{86.75} \small{$\pm$ 0.6} & \textbf{83.36 }\small{$\pm$ 0.6} \\
%     & \textbf{OAL-OFL-Lite}& 70.80 \small{$\pm$ 0.9} & 73.67 \small{$\pm$ 0.7} && \underline{86.66} \small{$\pm$ 0.6} & \underline{82.22} \small{$\pm$ 0.6} \\    
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{-0.5cm}
% \end{table*}


\noindent\textbf{Evaluation protocol.} 
We use the predicted probability for $(N+1)$th class as an open-set score and report threshold-free measurement AUROC~\cite{AUROC, AUROC2}. 
% The prediction for closed-set classification is decided by selecting the class with the highest probability among closed-set categories. We report closed-set results in terms of top-1 accuracy.
For closed-set evaluation, we predict the class with the highest probability among closed-set categories and report top-1 accuracy (Acc). % \kh

\noindent \textbf{Compared methods.} We conduct a comparative analysis of our OAL-OFL method against various existing approaches, encompassing both FSL methods such as~\cite{protonet, FEAT} and FSOSR methods~\cite{PEELER, snatcher_cvpr21, TANE, GEL}.


 %\textbf{ASOP (Ours)} & 66.30 \small{$\pm$ 0.6} & \underline{71.72} \small{$\pm$ 0.5} && \underline{82.68 \small{$\pm$ 0.2}} & \underline{80.92 \small{$\pm$ 0.2}} && 68.68 \small{$\pm$0.7} & {74.92 \small{$\pm$ 0.4}} && 84.84 \small{$\pm$ 0.4} & \textbf{82.37 \small{$\pm$ 0.3}} \\ % 0.1, 0.5, 0.4
    
    %\textbf{ASOP-L (Ours)} & \textbf{67.85 \small{$\pm$ 0.2}} & \textbf{71.91 \small{$\pm$ 0.7}} && \textbf{82.81 \small{$\pm$ 0.3}} & \textbf{81.04 \small{$\pm$ 0.2}} && \textbf{71.49} \small{$\pm$ 0.4} & \textbf{75.04} \small{$\pm$ 0.4} && \underline{85.15} \small{$\pm$ 0.1} & 81.51 \small{$\pm$ 0.1}\\
    %\textbf{Stage-1} & 67.95 & 71.81 && 82.76 & 80.91 && 71.17 & 74.57 && 84.75 & 81.34 \\



\begin{comment}
\begin{table}[t]
    \caption{
    \textbf{Comparative results on the \textit{mini}ImageNet and \textit{tiered}ImageNet.} Averages of Acc (\%) and AUROC (\%) over 600 tasks are reported with 95\% confidence interval (*: reproduced numbers, ${}^{\dagger}$: results from \cite{snatcher_cvpr21}). For each case, bold and underlined scores indicate the best and second-best results.}
    % \vspace{-0.2cm}
    \label{table:main_result}
    \centering
    \renewcommand{\arraystretch}{1.0}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    
    \multirow{2}{*}{\textbf{Methods}} &\multicolumn{2}{c}{\textbf{1-shot}} && \multicolumn{2}{c}{\textbf{5-shot}}\\
    \cmidrule{2-3} \cmidrule{5-6}
    & Acc. & AUROC && Acc. & AUROC\\
    \midrule
    \midrule
    \multicolumn{6}{c}{\textit{mini}ImageNet}\\
    \midrule
    ProtoNets\cite{protonet}${}^{\dagger}$ & 64.01 \small{$\pm$ 0.9} & 51.81 \small{$\pm$ 0.9} && 80.09 \small{$\pm$ 0.6} & 60.39 \small{$\pm$ 0.9} \\
    FEAT~\cite{FEAT}${}^{\dagger}$ & 67.02 \small{$\pm$ 0.9} & 57.01 \small{$\pm$ 0.8} && 82.02 \small{$\pm$ 0.5} & 63.18 \small{$\pm$ 0.8}\\
    PEELER~\cite{PEELER}${}^{\dagger}$ & 65.86 \small{$\pm$ 0.9} & 60.57 \small{$\pm$ 0.8} && 80.61 \small{$\pm$ 0.6} & 67.35 \small{$\pm$ 0.8}\\
    SnaTCHer-F~\cite{snatcher_cvpr21} & 67.02 \small{$\pm$ 0.9} & 68.27 \small{$\pm$ 1.0} && 82.02 \small{$\pm$ 0.5} & 77.42 \small{$\pm$ 0.7}\\
    SnaTCHer-T~\cite{snatcher_cvpr21} & 66.60 \small{$\pm$ 0.8} & 70.17 \small{$\pm$ 0.9}&&81.77 \small{$\pm$ 0.5} &76.66 \small{$\pm$ 0.8}\\
    SnaTCHer-L~\cite{snatcher_cvpr21} & 67.60 \small{$\pm$ 0.8}&69.40 \small{$\pm$ 0.9}&&82.36 \small{$\pm$ 0.6} &76.15 \small{$\pm$ 0.8}\\
    ATT~\cite{TANE} & 67.64 \small{$\pm$ 0.8} & 71.35 \small{$\pm$ 0.7} && 82.31 \small{$\pm$ 0.5} & 79.85 \small{$\pm$ 0.6}\\
    ATT-G~\cite{TANE} & 68.11 \small{$\pm$ 0.8} & 72.41 \small{$\pm$ 0.7} && 83.12 \small{$\pm$ 0.5} & 79.85 \small{$\pm$ 0.6}\\
    GEL~\cite{GEL} & 68.26 \small{$\pm$ 0.9} & \underline{73.70} \small{$\pm$ 0.8} && 83.05 \small{$\pm$ 0.6} & \underline{82.29} \small{$\pm$ 0.6} \\
    
    \cmidrule{1-6}
   
    \textbf{OAL-OFL} & \textbf{69.78} \small{$\pm$ 0.8} & \textbf{73.88} \small{$\pm$ 0.7} && \underline{85.49} \small{$\pm$ 0.7} & \textbf{83.13} \small{$\pm$ 0.6}\\
    
    \textbf{OAL-OFL-Lite} & \underline{69.15} \small{$\pm$ 0.8} & 72.21 \small{$\pm$ 0.9} && \textbf{85.61} \small{$\pm$ 0.6} & 81.11 \small{$\pm$ 0.6}\\    
    
    % \textbf{ASOP-F (Ours)} & 67.23 \small{$\pm$ 0.6} & 72.02 \small{$\pm$0.3} && 82.60 \small{$\pm$0.2} & 81.69 \small{$\pm$0.4}\\

    
    \midrule
    \midrule
    \multicolumn{6}{c}{\textit{tiered}ImageNet}\\
    \midrule
    ProtoNets\cite{protonet}${}^{\dagger}$& 68.26 \small{$\pm$ 1.0} & 60.73 \small{$\pm$ 0.8} && 83.40 \small{$\pm$ 0.7} & 64.96 \small{$\pm$ 0.8}  \\
    FEAT~\cite{FEAT}${}^{\dagger}$ & 70.52 \small{$\pm$ 1.0} & 63.54 \small{$\pm$ 0.7} && 84.74 \small{$\pm$ 0.7} & 70.74 \small{$\pm$ 0.8}\\
    PEELER~\cite{PEELER}${}^{\dagger}$ & 69.51 \small{$\pm$ 0.9} & 65.20 \small{$\pm$ 0.8} && 84.10 \small{$\pm$ 0.7} & 73.27 \small{$\pm$ 0.7}\\
    SnaTCHer-F~\cite{snatcher_cvpr21} & 70.52 \small{$\pm$ 1.0} & 74.28 \small{$\pm$ 0.8} && 84.74 \small{$\pm$ 0.7} & 82.02 \small{$\pm$ 0.6}\\
    SnaTCHer-T~\cite{snatcher_cvpr21} & 70.45 \small{$\pm$ 1.0} & 74.84 \small{$\pm$ 0.8} && 84.42 \small{$\pm$ 0.7} & 82.03 \small{$\pm$ 0.7} \\
    SnaTCHer-L~\cite{snatcher_cvpr21} & \underline{70.85} \small{$\pm$ 1.0} & 74.95 \small{$\pm$ 0.8} && 85.23 \small{$\pm$ 0.6} & 80.81 \small{$\pm$ 0.7}\\
    ATT~\cite{TANE} & 69.34 \small{$\pm$ 1.0} & 72.74 \small{$\pm$ 0.8} && 83.82 \small{$\pm$ 0.6} & 78.66 \small{$\pm$ 0.7}\\
    ATT-G~\cite{TANE} & 70.58 \small{$\pm$ 0.9} & 73.43 \small{$\pm$ 0.8} && 85.38 \small{$\pm$ 0.6} & 81.64 \small{$\pm$ 0.6}\\
    GEL~\cite{GEL} & 70.50 \small{$\pm$ 0.9} & \underline{75.86} \small{$\pm$ 0.8} && 84.60 \small{$\pm$ 0.7} & 81.95 \small{$\pm$ 0.7} \\
    \cmidrule{1-6}
    \textbf{OAL-OFL} & \textbf{71.73 }\small{$\pm$ 0.5}  & \textbf{75.88 }\small{$\pm$ 0.6} && \textbf{86.75} \small{$\pm$ 0.6} & \textbf{83.36 }\small{$\pm$ 0.6} \\
    \textbf{OAL-OFL-Lite}& 70.80 \small{$\pm$ 0.9} & 73.67 \small{$\pm$ 0.7} && \underline{86.66} \small{$\pm$ 0.6} & \underline{82.22} \small{$\pm$ 0.6} \\    
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.5cm}
\end{table}
\end{comment}
% \vspace{-0.15cm}
\subsection{Comparative Assessment}
\vspace{-0.2cm}
Table~\ref{table:main_result} presents a comparison between our OAL-OFL and baselines in 5-way \{1, 5\}-shot settings on \textit{mini}ImageNet and \textit{tiered}ImageNet. FSL approaches~\cite{protonet, FEAT} were not designed for FSOSR, we applied them to FSOSR in a straightforward manner as in \cite{snatcher_cvpr21}. In brief, in the FSL methods, the open-set detection score is computed by taking the negative of the largest classification probability~\cite{ODIN}. Compared to the FSOSR methods, PEELER, SnaTCHers and ATT, both OAL-OFL and OAL-OFL-Lite show better generalized capabilities, as reflected by their Acc and AUROC across datasets.

Nevertheless, notice that there has been no further performance improvement since GEL, highlighting the challenges of progress in FSOSR. This is largely due to the inherent trade-off between Acc and AUROC—two metrics that often conflict. For instance, although GEL achieves the best AUROC among prior methods, it falls short of ATT-G in terms of Acc across both 1 and 5-shot settings.
%The objective of FSOSR is to excel in open-set recognition while simultaneously maintaining high closed-set accuracy. Whereas prior methods have predominantly concentrated on open-set recognition, our approach has demonstrated significant improvements in closed-set accuracy, showcasing clear advantages over these earlier techniques. Notice that there has been no further performance improvement since GEL, highlighting the challenges of progress in FSORS. FSOSR requires balancing both Acc and AUROC, which often conflict with each other. For example, even GEL attains the best AUROC in prior methods, but it falls short of ATT-G for Acc across both 1 and 5-shot settings.
More specifically, it is observed that the previous approaches exhibit a particular bias towards miniImageNet. ATT-G improves ATT by using the base class prototypes to enhance closed-set prototypes. Nevertheless, it is even worse than our OAL-OFL-Lite which does not use the base training dataset. GEL makes predictions for both pixel-wise and semantic-wise by adding a 2D convolutional block on top of the SnaTCHer-F. It attained the previous SOTA in \textit{mini}ImageNet, but not in all measures. Whereas we achieve SOTA performance \textit{in all cases}. In 1-shot setting, we slightly outperform GEL in AUROC, but are much better in Acc (1.52\% in \textit{mini}ImageNet and 1.23\% in \textit{tiered}ImageNet). Notice that in FSOSR, both closed-set classification and open-set detection are important. In 5-shot setting, our method shows clear SOTA performance in both Acc and AUROC. In specific, 2.59\% Acc and 0.84\% AUROC in \textit{mini}ImageNet, and 2.15\% Acc and 1.41\% in \textit{tiered}ImageNet. Namely, when only a few examples per class are increased (one to five), the proposed \jt{open-set free} transfer learning more faithfully makes it beneficial. Also, even without the base training dataset, OAL-OFL-Lite surpasses or is comparable to the existing FSOSR methods in both datasets. Therefore, we conclude that our two-stage approach successfully pioneers transfer learning for FSOSR. In addition, cross-domain comparative results are provided in Appendix.



\begin{comment}
\begin{table}[t]
\caption{\textbf{Difficulty of transfer learning in FSOSR}. %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
}
\label{table:difficulty}
\vspace{-0.3cm}
\centering
\resizebox{0.9\linewidth}{!}
{
    \begin{tabular}{cccccc}
    \toprule
    %\multirow{2}{*}{Stage-1}& \multirow{2}{*}{Stage-2} & \multirow{2}{*}{$\mathcal{L}^2_{\textrm{KL}}$ in Stage-2}& \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    %\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
    \cmidrule{2-3} \cmidrule{5-6}
    %& $\mathcal{L}^2_{\textrm{KL}}$ & $[a, b]$ && Acc. & AUROC && Acc. & AUROC\\
     & Acc. & AUROC && Acc. & AUROC\\
    \midrule
    \midrule
    %& & &   &  &&  & \\
    %\multicolumn{2}{c}{Naive TL to closed set} &  66.05 & 62.38 && 84.21 & 69.07 \\
    Naive TL to closed set & 66.05 & 62.38 && 84.21 & 69.07 \\ 
    Stage-2 only + regul. &  56.97 & 67.78 && 78.98 & 76.72 \\
    \midrule
    \textbf{OFL (Stage-2 only)} & 56.72 & 67.47 && 78.59 & 76.64 \\
    \textbf{OAL-OFL} & \textbf{69.78}& \textbf{73.88}&& \underline{85.49} & \textbf{83.13}\\
    
    \bottomrule
    \end{tabular}
}
% \vspace{-0.4cm}
\end{table}
\end{comment}



\begin{table}[t]
\caption{\textbf{Ablation analysis on stages in the proposed OAL-OFL}. %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
}
\label{table:stage_ablation}
\centering
\resizebox{0.55\linewidth}{!}
{
    \begin{tabular}{ccccccc}
    \toprule
    %\multirow{2}{*}{Stage-1}& \multirow{2}{*}{Stage-2} & \multirow{2}{*}{$\mathcal{L}^2_{\textrm{KL}}$ in Stage-2}& \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \multirow{2}{*}{Stage-1}& \multirow{2}{*}{Stage-2} & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    %\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
    \cmidrule{3-4} \cmidrule{6-7}
    %& $\mathcal{L}^2_{\textrm{KL}}$ & $[a, b]$ && Acc. & AUROC && Acc. & AUROC\\
    & & Acc. & AUROC && Acc. & AUROC\\
    \midrule
    \midrule
    %& & &   &  &&  & \\
    \multicolumn{2}{c}{Naive TL to closed set} &  66.05 & 62.38 && 84.21 & 69.07 \\
    \multicolumn{2}{c}{Stage-2 only + regul.} &  56.97 & 67.78 && 78.98 & 76.72 \\

    \midrule
    
    %\multicolumn{2}{c}{\jt{Baseline}} & 67.60 & 69.40 && 82.36 & 76.15\\
     & $\checkmark$ & 56.72 & 67.47 && 78.59 & 76.64 \\
    %$\checkmark$&  &  & 67.95 & 71.81 && 82.76 & 80.91  \\
    $\checkmark$&  &  67.95 & 71.81 && 82.76 & 80.91  \\
    %$\checkmark$ & $\checkmark$ &  & 67.68 & 70.64 && 83.51 & 80.37 \\
    %$\checkmark$ & $\checkmark$ &  & 69.07 & 71.38 && 84.12 & 82.09 \\
    %$\checkmark$ & $\checkmark$ & $\checkmark$ & 69.43 & 73.40 && 85.18 & 82.75 \\
    % \midrule
    $\checkmark$ & $\checkmark$ & 69.78 & 73.88 && 85.49 & 83.13 \\
    % \checkmark & \checkmark & \checkmark & \checkmark & \textbf{66.3} & \textbf{71.8} && 82.6 & 80.7 \\
    
    \bottomrule
    \end{tabular}
}
\vspace{-0.4cm}
\end{table}




%the 1st stage is critical for transfer learning in FSOSR setting.

\begin{figure*}[t]
  \centering
   %\subfigure[OAL-OFL] {\includegraphics[width=8.5cm]{Figure/Iter_OAL-OFL.png}}\;\;
    %\subfigure [OAL-OFL-lite (TBU)] {\includegraphics[width=8.5cm]{Figure/Iter_OAL-OFL.png}}
   \subfloat[Stage-1 only] {\includegraphics[width=4.2cm]{Figure/hist3_st1.png}} \quad
   \subfloat[Stage-2 only] {\includegraphics[width=4.2cm]{Figure/hist3_st2.png}} \quad
   \subfloat[OAL-OFL] {\includegraphics[width=4.2cm]{Figure/hist3_ltl.png}} \quad
   %\subfigure {\includegraphics[width=3.6cm]{Figure/tsne_legend.png}}
  \caption{\textbf{Distribution of the classification probabilities of closed-set and open-set queries to the open-set class.} Closed-set and open-set queries are represented in green and red, respectively.}
  \label{fig:hist}
  \vspace{-0.5cm}
\end{figure*}


\vspace{-0.15cm}
\subsection{Analysis}
\vspace{-0.25cm}
We extensively analyze the proposed method on \textit{mini}ImageNet. More analyses are in the Appendix.
% particularly with regard to OAL-OFL-Lite.

\noindent\textbf{Difficulty of TL in FSOSR.} \jtt{To see the efficacy of the respective stage of our method especially in FSOSR, we first analyze the proposed OAL-OFL comparing with two straightforward transfer learning schemes in Table~\ref{table:stage_ablation}. First, in `Naive TL to closed set' of the first row, we conduct a naive transfer learning~\cite{IER_distill} without the base training dataset. Namely, the model is fit to $N$-way closed-set classification through linear regression~\cite{chencloser}, and rejects the open-set queries thresholding max-probability~\cite{openmax}. This naive approach shows severely low performance, which indicates the difficulty of FSOSR transfer learning.
Second, in `Stage-2 only + regul.,' the pseudo-label-based regularization exploits the base training dataset to compute the Kullback–Leibler divergence between the pre-trained model and transfer-learned model, which showed promising results in transfer learning for FSL~\cite{fsl_halluc}. Skipping Stage-1, we can apply this regularization technique during transfer learning which is `Stage-2 only + regul.' This approach (single-stage + regularization) shows only slight improvement compared to the case of only Stage-2 (1st row of the lower part of  Table~\ref{table:stage_ablation}). Whereas, our OAL-OFL achieves meaningful transfer learning results by combining the two stages.}

%\subsubsection{\bg{OAL-OFL (Stage-2 with $\mathcal{D}_\rmbase$})}
\noindent\textbf{Two-stage training (OAL-OFL).
% (w/ $\mathcal{D}_\rmbase$).
} To demonstrate the impact of the proposed two-stage training approach, we first ablate the stages in Table~\ref{table:stage_ablation} for OAL-OFL. When Stage-1 is skipped, the open-set classifier $w_{N+1}$, and scalars ($a,b$) are initialized in random and (1,0), respectively in Stage-2. Relying solely on Stage-2 causes overfitting to the training examples. Then, %compared to the baseline (the first row of Table~\ref{table:stage_ablation}), 
it leads to highly degenerated results of 56.72\% and 78.59\% for 1- and 5-shot closed-set classification Acc, respectively, and 67.47\% and 76.64\% for 1- and 5-shot open-set detection AUROC, respectively. These results highlight that the \jt{open-set aware} meta-learning of Stage-1 is critical for the success of transfer learning in FSOSR.  %Next, Stage-1 alone can attain a decent performance which is slightly better than the baseline. 



Notice that, in ATT-G~\cite{TANE}, the base training dataset calibrates the closed-set classifiers even in testing phase, but it marginally improves ATT~\cite{TANE} (see Table~\ref{table:main_result}). Whereas, in the proposed OAL-OFL, the use of the base training dataset during the \jt{open-set free} training of Stage-2 gives notable improvement. Applied on top of Stage-1, Stage-2 attains notably improved results by 1.83\% and 2.70\% in Acc, and 2.07\% and 2.22\% in AUROC for 1- and 5-shot respectively. 
%These results highlight that a favorably meta-learned model is critical for the success of transfer learning in FSOSR. 

In Fig.~\ref{fig:hist}, we present a visualization of the distributions of classification probability towards the open-set class, derived from both closed-set and open-set queries. The visualization reveals that, in the scenario labeled as `Stage-2 only,' where the open-set aware meta-learning is absent, a majority of the queries are assigned high probabilities of belonging to the open-set, irrespective of their actual membership to the closed or open set. Converserly, in `Stage-1 only' scenario, a significant number of closed-set queries are still attributed probabilities exceeding 0.5. On the other hand, in OAL-OFL, it is observed that the majority of open-set queries attain significantly high probabilities of being classified as the open-set, while the probabilities for closed-set queries are effectively suppressed. This distinct separation in the classification probabilities for open and closed-set queries allows us to understand and verify the robustness of OAL-OFL in dichotomizing between open and closed sets.
  

%\add{Next, to see the efficacy of Stage-1 further, we can also compare our OAL-OFL with single-stage transfer learning with the regularization technique. The pseudo-label-based regularization exploits the base training dataset to compute the Kullback–Leibler divergence between the pre-trained model and transfer-learned model, which showed promising results in transfer learning for FSL~\cite{fsl_halluc}. Skipping Stage-1, we apply this regularization technique during transfer learning which is `Stage-2 only + regul.' This approach (single-stage + regularization) shows only slight improvement compared to the case of only Stage-2 (1st row of Table~\ref{table:stage_ablation}). Whereas, our OAL-OFL achieves meaningful transfer learning results by introducing the Stage-1.}


\begin{comment}
\begin{table}[t]
\caption{\textbf{Ablation analysis for our OAL-OFL-Lite in Stage-2.} %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
}
\label{table:stage2_ablation_lite}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{0.65\linewidth}{!}
{
    \begin{tabular}{ccccccc}
    \toprule
    \multirow{2}{*}{}& \multirow{2}{*}{} & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    %\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
    \cmidrule{3-4} \cmidrule{6-7}
    & & Acc. & AUROC && Acc. & AUROC\\
    \midrule
    \midrule
    \multicolumn{2}{c}{Naive TL to closed set} & 66.05 & 62.38 && 84.21 & 69.07 \\ 
    \multicolumn{2}{c}{Stage-2 only} & 57.72 & 68.13 && 78.43 & 79.36 \\ 
    % \multicolumn{2}{c}{Stage-2 + regul.} &  56.97 & 67.78 && 78.98 & 76.72 \\
    \multicolumn{2}{c}{OAL-OFL-Lite} &  69.15 & 72.21 && 85.61 & 81.11   \\ 
    \midrule
    \midrule
    Pseudo open set & Freeze $w_{N+1}$ & &  &&  &  \\     
    \midrule    
    & & 68.14 & 71.52 && 84.36 & 80.88 \\     
    % & $\checkmark$ & 67.38 & 71.11 && 84.50 & 80.63 \\
    $\checkmark$&  &  68.20 & 71.33 && 85.12 & 80.61  \\
    $\checkmark$ & $\checkmark$ & 69.15 & 72.21 && 85.61 & 81.11 \\
    \bottomrule
    \end{tabular}
}
\vspace{-0.5cm}
\end{table}
\end{comment}

\begin{table}[t]
\caption{\textbf{Ablation analysis for our OAL-OFL-Lite in Stage-2.} %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
}
\label{table:stage2_ablation_lite}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}
{
    \begin{tabular}{ccccccc|ccccccc}
    \toprule
    \multirow{2}{*}{}& \multirow{2}{*}{} & \multicolumn{2}{c}{1-shot} & \multicolumn{2}{c}{5-shot} && &\multirow{2}{*}{\shortstack{Pseudo\\\newline open set}} & \multirow{2}{*}{\shortstack{Freeze\\\newline $w_{N+1}$}}& \multicolumn{2}{c}{1-shot} & \multicolumn{2}{c}{5-shot}\\
    %\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
    \cmidrule{3-4} \cmidrule{5-6} \cmidrule{11-12} \cmidrule{13-14}
    & & Acc. & AUROC & Acc. & AUROC &&  && & Acc. & AUROC & Acc.  & AUROC \\ 
    \midrule
    \midrule
     %& & & & & & & Pseudo open set & Freeze $w_{N+1}$ & &  &&  &  \\ 
    \multicolumn{2}{c}{Naive TL to closed set} & 66.05 & 62.38 & 84.21 & 69.07 && \multirow{3}{*}{\shortstack{OAL-OFL\\\newline-Lite}}  & & & 68.14 & 71.52 & 84.36 & 80.88 \\      
    \multicolumn{2}{c}{Stage-2 only} & 57.72 & 68.13 & 78.43 & 79.36 && &$\checkmark$&  &  68.20 & 71.33 & 85.12 & 80.61  \\
    % \multicolumn{2}{c}{Stage-2 + regul.} &  56.97 & 67.78 && 78.98 & 76.72 \\
    \multicolumn{2}{c}{OAL-OFL-Lite} &  69.15 & 72.21 & 85.61 & 81.11 && &$\checkmark$ & $\checkmark$ & 69.15 & 72.21 & 85.61 & 81.11 \\
    %\midrule
    %\midrule
    %Pseudo open set & Freeze $w_{N+1}$ & &  &&  &  \\     
    %\midrule    
    
    % & $\checkmark$ & 67.38 & 71.11 && 84.50 & 80.63 \\
    
    %
    \bottomrule
    \end{tabular}
}
\vspace{-0.4cm}
\end{table}


%\section{The Distribution of classification probability assigned to the open-set class}



%The first row of Table~\ref{table:stage_ablation} shows that relying solely on Stage-2 leads to highly degenerated results of 56.72\% and 78.59\% for 1- and 5-shot closed-set classification accuracy, respectively, and 67.47\% and 76.64\% for 1- and 5-shot open-set detection AUROC, respectively. Next, in the second row, Stage-1 alone can attain a decent performance which is slightly better than the existing SOTA~\cite{TANE}. Applied on top of Stage-1, Stage-2 attains significantly improved results by \jt{1.83\%} and \jt{2.70\%} in accuracy, and \jt{2.07\%} and \jt{2.22\%} in AUROC for 1- and 5-shot respectively. %These results highlight that a favorably meta-learned model is critical for the success of transfer learning in FSOSR. 

\noindent\textbf{Two-stage training (OAL-OFL-Lite).} The left part of Table~\ref{table:stage2_ablation_lite} shows the stage ablation for OAL-OFL-Lite. 
% Since the same Stage-1 model is exploited for OAL-OFL and OAL-OFL-Lite, we skip the analysis on Stage-1 here.
On top of the same Stage-1 model of OAL-OFL, the open-set free transfer learning of OAL-OFL-Lite also achieves a notable improvement on the Stage-1 model in Table~\ref{table:stage_ablation}. As shown in the ablation study on OAL-OFL, `Stage-2 only' results in a large performance drop compared to the OAL-OFL-Lite of the third row. In the following sections, we study the key components of the \jt{open-set free} transfer learning of the proposed OAL-OFL and OAL-OFL-Lite.
% Further, 


% \begin{table}[t]
% \caption{\textbf{Two-stage transfer learning (our OAL-OFL) \textit{vs.} single stage transfer learning with regularization}.}
% \label{table:regul}
% \vspace{-0.2cm}
% \centering
% \renewcommand{\arraystretch}{1.1}
% \resizebox{\linewidth}{!}
% {
%     \begin{tabular}{cccccc}
%     \toprule
%      & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
%     \cmidrule{2-3} \cmidrule{5-6}
%     Transfer learning &Acc. & AUROC && Acc. & AUROC \\
%     \midrule
%     \midrule
%     Single-stage + regul. &  56.97 & 67.78 && 78.98 & 76.72 \\
%     Two-stage (OAL-OFL) & 69.78 & 73.88 && 85.49 & 83.13\\
%     \bottomrule
%     \end{tabular}
% }
% \end{table}


%In `Naive TL to closed set' of the first row, we show a naive transfer learning~\cite{IER_distill} without the base training dataset. Namely, the model is fit to $N$-way closed-set classification through linear regression~\cite{chencloser}, and rejects the open-set queries thresholding max-probability~\cite{openmax}. The naive approach shows severely low performance, which indicates the difficulty of FSOSR transfer learning. In the second row, as in OAL-OFL, `Stage-2 only' results in a large performance drop compared to the OAL-OFL-Lite of the third row. In the following sections, we study the key components of the \jt{open-set free} transfer learning of the proposed OAL-OFL and OAL-OFL-Lite.

\noindent\textbf{Pseudo open set \& Frozen $w_{N+1}$.} OAL-OFL-Lite deals with the challenge of the absence of the base training dataset by the episodic sampling of the pseudo open set and freezing $w_{N+1}$. The right part of Table~\ref{table:stage2_ablation_lite} shows the importance of the two components. Without both (the first row), the model focuses on learning closed-set classification, showing better Acc and lower AUROC than using only Stage-1 in Table~\ref{table:stage_ablation}. Although the pseudo open-set sampling is used, transfer learning the open-set classifier is still challenging as demonstrated in the second row. Hence, as in the last row, we freeze the open-set classifier and perform episodic pseudo open-set sampling.

\begin{figure}[t]
  \centering
   %\subfigure[OAL-OFL] {\includegraphics[width=8.5cm]{Figure/Iter_OAL-OFL.png}}\;\;
    %\subfigure [OAL-OFL-lite (TBU)] {\includegraphics[width=8.5cm]{Figure/Iter_OAL-OFL.png}}
    \begin{subfigure}{0.49\linewidth}\includegraphics[width=\linewidth]{Figure/Iter_1shot_v6.png}
    \caption{5-way 1-shot}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}\includegraphics[width=\linewidth]{Figure/Iter_5shot_v6.png}
    \caption{5-way 5-shot}
    \end{subfigure}
  \caption{\textbf{Plots of OAL-OFL on Acc (\%), AUROC (\%), and loss (logarithmic scale) on iterations in Stage-2} (Best viewed in color).} %on the 5-way 1- and 5-shot settings of the \textit{mini}ImageNet. }
  \label{fig:iters}
\vspace{-0.5cm}
\end{figure}

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{minipage}{0.48\linewidth}
    \centering
    \caption{\textbf{Ablation analysis for Stage-1.}}
    \label{table:st1_ablation}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccccc}
        \toprule
        &&\multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
        \cmidrule{3-4} \cmidrule{6-7}
        $\mathcal{L}_\textrm{mask}^1$ & $(a,b)$ & Acc. & AUROC && Acc. & AUROC\\
        \midrule
        \midrule
         & & 66.07 & 70.72 && 82.01 & 80.14  \\
        $\checkmark$ & & 66.45 & 71.06 && 81.75 & 80.31 \\
        $\checkmark$ & $\checkmark$ & 67.95 & 71.81 && 82.76 & 80.91 \\
        % \checkmark & \checkmark & \checkmark & \checkmark & \textbf{66.3} & \textbf{71.8} && 82.6 & 80.7 \\
        \bottomrule
        \end{tabular}
    }
    
\end{minipage}%
\hfill%
\begin{minipage}{0.48\linewidth}
    \centering
    \caption{\textbf{Impact of the base training dataset varying the number of classes in Stage-2.} %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
    }
    \label{table:vary_basedata}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccc}
        \toprule
        & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
        \cmidrule{2-3} \cmidrule{5-6}
        \#Base categories &Acc. & AUROC && Acc. & AUROC \\
        \midrule
        \midrule
        0 (OAL-OFL-Lite) & 69.15 & 72.71 && 85.61 & 81.11\\
        \midrule
        1 & 66.41 & 69.62 && 83.66 & 79.62 \\
        6 & 66.72 & 69.71 && 83.15 & 78.34 \\
        32 & 68.30 & 71.84 && 84.51 & 81.34\\
        64 (OAL-OFL) & 69.78 & 73.88 && 85.49 & 83.13\\

        \bottomrule
        \end{tabular}
    }
    
\end{minipage}
\vspace{-0.4cm}
\end{table}

\noindent\textbf{Stage-1 to prevent overfitting.
% (w/ $\mathcal{D}_\rmbase$).
}
% Fig.~\ref{fig:iters} measures the performance increasing the iterations in Stage-2 of OAL-OFL.
Fig.~\ref{fig:iters} visualizes the changes of Acc, AUROC, and loss values during Stage-2 training.
To see the impact of Stage-1 on Stage-2, we plot `Stage-2 only' and our complete OAL-OFL. 
Fig.~\ref{fig:iters}(a) right shows the loss curves. 
OAL-OFL starts from a pretty lower loss than `Stage-2 only.' And both `Stage-2 only' and OAL-OFL converge, but `Stage-2 only' is saturated at a higher loss. Also, OAL-OFL shows better performance over all the iterations in the testing ACC and AUROC of Fig.~\ref{fig:iters}(a) left. We can see a similar trend in 5-shot. From this result, we can infer that our Stage-1 can provide a favorable starting point, while mitigating the overfitting problem of FSOSR transfer learning.


%\begin{table*}[t]
%\centering%
%\renewcommand{\arraystretch}{1.1}


\begin{comment}
\begin{table}[t]
\caption{\textbf{Two-stage transfer learning (our OAL-OFL) \textit{vs.} single stage transfer learning with regularization}. %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
}
\label{table:regul}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}
{
    \begin{tabular}{cccccc}
    \toprule
     & \multicolumn{2}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \cmidrule{2-3} \cmidrule{5-6}
    Transfer learning &Acc. & AUROC && Acc. & AUROC \\
    \midrule
    \midrule
    %Linear & 63.11 & 70.64 && 83.41 & 80.33 \\
    Single-stage + regul. &  56.97 & 67.78 && 78.98 & 76.72 \\
    %Euclidean & 68.56 & 72.17 && 84.39 & 82.52\\
    Two-stage (OAL-OFL) & 69.78 & 73.88 && 85.49 & 83.13\\
    \bottomrule
    \end{tabular}
}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[t]
\caption{\textbf{Ablation analysis for Stage-1.}}
\label{table:st1_ablation}
\centering
\resizebox{0.52\linewidth}{!}
{
    \begin{tabular}{ccccccc}
    \toprule
    &&\multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \cmidrule{3-4} \cmidrule{6-7}
    $\mathcal{L}_\textrm{mask}^1$ & $(a,b)$ & Acc. & AUROC && Acc. & AUROC\\
    \midrule
    \midrule
     & & 66.07 & 70.72 && 82.01 & 80.14  \\
     $\checkmark$ & & 66.45 & 71.06 && 81.75 & 80.31 \\
     $\checkmark$ & $\checkmark$ & 67.95 & 71.81 && 82.76 & 80.91 \\
    % \checkmark & \checkmark & \checkmark & \checkmark & \textbf{66.3} & \textbf{71.8} && 82.6 & 80.7 \\
    \bottomrule
    \end{tabular}
}
\vspace{-0.3cm}
\end{table}
\end{comment} 
%%%%


\noindent\textbf{Analysis on Stage-1.}
We exploited the scalar factors, $a$ and $b$, and masked loss $L_\textrm{mask}$ to facilitate learning task-independent open-set prototype in the meta-learning of Stage-1. Table~\ref{table:st1_ablation} ablates these components. All the components are useful, and the degraded performance in the ablated ones means the difficulty of meta-learning the task-independent open-set prototype.

%From this, we identified the importance of the meta-learning stage to mitigate overfitting in FSOSR transfer learning. 
\begin{comment}
To see the effectiveness of Stage-1 further, we can also compare OAL-OFL (two-stage transfer learning) with single-stage transfer learning with the regularization technique to reduce the overfitting problem. The pseudo-label-based regularization~\cite{fsl_halluc} exploits the base training dataset to compute the Kullback–Leibler divergence between the pre-trained model and transfer-learned model, which showed promising results in transfer learning of few-shot classification. Instead of skipping Stage-1, we can apply this regularization technique during transfer learning. As in Table~\ref{table:regul}, this approach  (single-stage + regularization) is worse compared to `Stage-2 only' of Table~\ref{table:stage_ablation}. Whereas, our two-stage approach achieves meaningful transfer learning results.
    
\end{comment}
% This result demonstrates the difficulty of transfer learning of FSOSR.



%\noindent\textbf{Meta-learning \textit{vs.} regularization.} \jt{We compare it with the transfer learning with the base data regularization technique~\cite{fsl_halluc} where the output from an FSL pre-trained model is used for pseudo labels of transfer-learned model's predictions for the base training dataset. This regularization technique has shown promising results in FSL, the transfer-learned model is degenerated in FSOSR as in Table xxx.}

%\noindent\textbf{Metric space visualization.}
% (w/ $\mathcal{D}_\rmbase$).



\begin{comment}
\begin{table}[t]
\caption{\textbf{Impact of the base training dataset varying the number of classes in Stage-2.} %Accuracy (\%) and AUROC (\%) are reported on the 5-way 1- and 5-shot settings on the \textit{mini}ImageNet.
}
\label{table:vary_basedata}
\centering
\resizebox{0.55\linewidth}{!}
{
    \begin{tabular}{cccccc}
    \toprule
     & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \cmidrule{2-3} \cmidrule{5-6}
    \#Base categories &Acc. & AUROC && Acc. & AUROC \\
    \midrule
    \midrule
    0 (OAL-OFL-Lite) & 69.15 & 72.71 && 85.61 & 81.11\\
    \midrule
    1 & 66.41 & 69.62 && 83.66 & 79.62 \\
    6 & 66.72 & 69.71 && 83.15 & 78.34 \\
    32 & 68.30 & 71.84 && 84.51 & 81.34\\
    64 (OAL-OFL) & 69.78 & 73.88 && 85.49 & 83.13\\
    
    \bottomrule
    \end{tabular}
}
\vspace{-0.3cm}
\end{table}
\end{comment}



\noindent\textbf{Amount of $\mathcal{D}_\rmbase$ in Stage-2.
% (w/ $\mathcal{D}_\rmbase$).
} 
% The various categories of base training dataset~$\mathcal{D}_\rmbase$ are not overlapped with those of $\mathcal{D}_\rmnew$, and hence can be used as the open-set training data in Stage-2 (w/ $\mathcal{D}_\rmbase$). 
In Table~\ref{table:vary_basedata}, we identify the impact of the variety of categories in $\mathcal{D}_\rmbase$ on the quality of the OFL. By reducing the number of categories in $\mathcal{D}_\rmbase$, the overall results are degraded. Rather, when the number of the base categories is lower than the half, OAL-OFL-Lite shows better results. Hence, it is crucial to configure the open-set training dataset from diverse base categories.

% Also, in the plot of Fig.~\ref{fig:iters}, the open-set training data are not redundantly sampled across iterations. Hence, more iterations mean more use of the base training dataset. We can see that the performance gets improved as the iteration increases. From these results, the large amount of base training dataset has a positive impact. And, potentially, we can expect more improvement if the higher quality base training dataset is given.

%\noindent\textbf{$\mathcal{L}_\textrm{KL}$ in Stage-2 (w/o $\mathcal{D}_\rmbase$).}




\begin{comment}
\begin{table}[t]
\caption{\textbf{Effect of meta-learning on the classifier of Stage-2}. (\sm{Rand}: random, \sm{Meta}: Stage-1 meta-learned).}
\label{table:init}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{0.8\linewidth}{!}
{
    \begin{tabular}{cccccccc}
    \toprule
     &\multicolumn{2}{c}{Classifier initialization} & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \cmidrule{4-5} \cmidrule{7-8}
    &$\{w_n\}_{n=1}^{N}$& $w_{N+1}$  &Acc. & AUROC && Acc. & AUROC \\
    \midrule
    \midrule
    %Linear & 63.11 & 70.64 && 83.41 & 80.33 \\
    \multirow{3}{*}{OAL-OFL-Lite} & \sm{Rand} & \sm{Rand} & 40.34 & 35.29 && 50.90 & 27.19 \\
    & \sm{Meta} & \sm{Rand} & 57.72 & 68.13 && 78.43 & 79.36\\
    %Euclidean & 68.56 & 72.17 && 84.39 & 82.52\\
    & \sm{Meta} & \sm{Meta} & 69.15 & 72.71 && 85.61 & 81.11\\
    \midrule
    \multirow{3}{*}{OAL-OFL} & \sm{Rand} & \sm{Rand} & 63.03  & 67.52 && 79.97 & 75.95 \\
    & \sm{Meta} & \sm{Rand} & 69.02 & 70.87 && 85.32 & 78.50 \\
    
    %Euclidean & 68.56 & 72.17 && 84.39 & 82.52\\
    & \sm{Meta} & \sm{Meta} & 69.78 & 73.88 && 85.49 & 83.13\\
    \bottomrule
    \end{tabular}
}
\end{table}
\end{comment}

\noindent\textbf{Meta-learned classifier.} In OAL-OFL and OAL-OFL-Lite, we utilize the meta-learned feature encoder and open-set prototype to initialize the closed-set and open-set classifiers. As in Table~\ref{table:init}, although the feature encoder starts from the meta-learned weights, the transfer-learned model suffers from severe performance degradation due to random initialization of both open and closed-set classifiers (Rand-Rand in Table~\ref{table:init}). In OAL-OFL, when the closed-set classifiers are initialized by the class-wise prototypes from the meta-learned encoder (Meta-Rand), the closed-set classification Acc is recovered, but open-set AUROC is not. In OAL-OFL-Lite, both Acc and AUROC are quite lower than the case of complete meta-learned weight initialization. Further, when both closed and open-set classifiers are not initialized by the meta-learned weight, the open-set recognition ability of OAL-OFL is worse than OAL-OFL-Lite where classifiers are initialized by the meta-learned weights. Hence, \jt{the open-set aware meta-learning} is crucial for the both closed- and open-set classifiers.

% \begin{comment}

% The linear one resulted in \jt{1.77\%} and \jt{0.77\%} decrease in 1 and 5-shot closed-set classification Acc, and \jt{1.09\%} and \jt{2.10\%} drop in 1 and 5-shot open-set AUROC. 
% These results 
% \end{comment}

%\subsubsection{\bg{OAL-OFL-Lite (Stage-2 without $\mathcal{D}_\rmbase$)}}


% \noindent\textbf{Other factors.} As presented in Table~\ref{table:loss_ablation}, the impact of the proposed regularization loss, $\mathcal{L}^2_\textrm{KL}$ and distance adjusting factors, $a$ and $b$, was analyzed. The purpose of $\mathcal{L}^2_\textrm{KL}$ is to mitigate overfitting~\cite{fsl_halluc}. The results show that the use of this regularization loss leads to 0.79\% and 0.43\% in 1-shot and 5-shot open-set AUROC, respectively. Additionally, the proposed distance adjusting factors, $a$ and $b$ produced notable improvements in both closed-set accuracy and open-set AUROC. These factors make it easier for a single open-set representation to satisfy desirable distances.

\begin{table}[t] % Use htbp for better float placement
\caption{\textbf{Effect of meta-learning on the classifier of Stage-2}. (\sm{Rand}: random, \sm{Meta}: Stage-1 meta-learned).}
\label{table:init} % Changed label
\centering
\renewcommand{\arraystretch}{1.1}
% Adjusted resizebox to 0.9\linewidth as the table is wider now (10 columns)
\resizebox{0.7\linewidth}{!}
{
    % cc (classifier init) + cccc (OAL-OFL-Lite) + cccc (OAL-OFL) = 10 columns
    \begin{tabular}{@{}cc cccc cccc@{}}
    \toprule
    % --- Header ---
    % Row 1: Method Names (Leave first 2 cols blank initially)
    \multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{OAL-OFL-Lite}} & \multicolumn{4}{c}{\textbf{OAL-OFL}} \\
    \cmidrule(lr){3-6} \cmidrule(lr){7-10} % Rules under method names
    % Row 2: Span "Classifier Initialization" upwards into blank cells of Row 1, add shot headers
    \multicolumn{2}{c}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Classifier\\Initialization\end{tabular}}}} & \multicolumn{2}{c}{\textbf{1-shot}} & \multicolumn{2}{c}{\textbf{5-shot}} & \multicolumn{2}{c}{\textbf{1-shot}} & \multicolumn{2}{c}{\textbf{5-shot}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} % Rules under shot counts
    % Row 3: Specific headers for initialization columns and metrics
    $\{w_n\}_{n=1}^{N}$ & $w_{N+1}$ & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC & Acc. & AUROC \\
    \midrule
    \midrule
    % --- Data Rows ---
    % Row 1: Rand / Rand initialization
    \sm{Rand} & \sm{Rand} & 40.34 & 35.29 & 50.90 & 27.19 & 63.03 & 67.52 & 79.97 & 75.95 \\
    % Row 2: Meta / Rand initialization
    \sm{Meta} & \sm{Rand} & 57.72 & 68.13 & 78.43 & 79.36 & 69.02 & 70.87 & 85.32 & 78.50 \\
    % Row 3: Meta / Meta initialization
    \sm{Meta} & \sm{Meta} & 69.15 & 72.71 & 85.61 & 81.11 & 69.78 & 73.88 & 85.49 & 83.13 \\
    \bottomrule
    \end{tabular}
}
\vspace{-0.4cm}
\end{table}

%\subsubsection{Cost for Stage-2}
\noindent\textbf{Cost for Stage-2.} As mentioned in Sec.~\ref{subsec:implementation}, we train the model with 20,000 tasks, an iteration per task in Stage-1. This is \textit{de facto} standard in FSOSR methods. In our Stage-2 of both OAL-OFL and OAL-OFL-Lite, the model is further learned during 300 iterations. It is only 1.5\% of Stage-1. While the model is not more generalized in Stage-1 with the 1.5\% additional iterations, our Stage-2 yields notable improvement as in Table~\ref{table:stage_ablation} through a tiny extra training cost.

% (Please refer to the Appendix for more analysis and the pseudo code.)

\begin{comment}
\begin{table}[t]
\caption{\textbf{Impact of the base training dataset varying the number of classes in Stage-2} Accuracy (\%) and AUROC (\%) on the \bg{5-way} 1- and 5-shot settings on the \textit{mini}ImageNet.}
\label{table:vary_basedata}
\centering
\resizebox{0.9\linewidth}{!}
{
    \begin{tabular}{cccccc}
    \toprule
     & \multicolumn{2}{c}{1-shot} && \multicolumn{2}{c}{5-shot}\\
    \cmidrule{2-3} \cmidrule{5-6}
    \#Base classes &Acc. & AUROC && Acc. & AUROC \\
    \midrule
    \midrule
    1 & 65.02 & 69.53 && 81.01 & 78.43 \\
    6 & 66.72 & 70.61 && 83.84 & 79.23\\
    32 & 68.11 & 71.69 && 84.80 & 82.38\\
    64 (Full) & 69.43 & 73.40 && 84.39 & 82.52\\
    \bottomrule
    \end{tabular}
}
\end{table}
\end{comment}

% \section{Discussions}
% %This work proposed a Learning to Transfer Learning (OAL-OFL), to address FSOSR via transfer learning. 
% % The results of OAL-OFL and OAL-OFL-Lite mean that transfer learning can be a powerful approach for FSOSR. Open-set sampling from the base training dataset yields the superior SOTA performance of OAL-OFL to OAL-OFL-Lite. For future investigation, we raise several discussion points to give valuable insights about this to the community.
% The results achieved with OAL-OFL and OAL-OFL-Lite demonstrate that transfer learning holds great potential for FSOSR. The superior performance of OAL-OFL over OAL-OFL-Lite can be attributed to open-set sampling from the base training dataset. As we consider future research directions, several discussion points come to the forefront:

% % (i) The performance suffers when there is a lack of the open-set data. OAL-OFL-Lite is effective in the extreme case (no access to the base training dataset), but it still freezes the open-set classifier in transfer learning. Future research could explore the better use of the limited open-set data.


% (i) The \bg{efficacy of OAL-OFL} can be negatively impacted \bg{with a scarcity of} open-set data. \bg{Although} OAL-OFL-Lite provides an effective solution in situations where the base training dataset is unavailable, it maintains the open-set classifier static \bg{throughout the transfer learning stage. Thus, there is an opportunity for future research to delve into methods for optimizing the use of pseudo} open-set data further refine the open-set classifier.

% (ii) \bg{In practical scenarios, it is often observed that the support examples gathered in testing environments are of sub-optimal quality. Moving forward, future research endeavors is expected to focus on addressing the complexities associated with FSOSR transfer learning, particularly under conditions where the support examples are disorganized. This includes scenarios where the examples originate from varied data distribution, rather than being derived from a unified, coherent dataset, and may even incorporate incorrectly labeled examples.}

==> arxiv2/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included the discussion section. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We described the method and datasets faithfully, and also included implementation details. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have described the implementation details %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provided the standard deviation for the results. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %$\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}%\answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%We used publicly available models and datasets, only %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included the discussion section. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We described the method and datasets faithfully, and also included implementation details. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have described the implementation details %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provided the standard deviation for the results. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %$\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}%\answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%We used publicly available models and datasets, only %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}
